Optimal Tree-Based Mechanisms for Differentially Private Approximate CDFs

This paper considers the $\varepsilon$-differentially private (DP) release of an approximate cumulative distribution function (CDF) of the samples in a dataset. We assume that the true (approximate) CDF is obtained after lumping the data samples into a fixed number $K$ of bins. In this work, we extend the well-known binary tree mechanism to the class of \emph{level-uniform tree-based} mechanisms and identify $\varepsilon$-DP mechanisms that have a small $\ell_2$-error. We identify optimal or close-to-optimal tree structures when either of the parameters, which are the branching factors or the privacy budgets at each tree level, are given, and when the algorithm designer is free to choose both sets of parameters. Interestingly, when we allow the branching factors to take on real values, under certain mild restrictions, the optimal level-uniform tree-based mechanism is obtained by choosing equal branching factors \emph{independent} of $K$, and equal privacy budgets at all levels. Furthermore, for selected $K$ values, we explicitly identify the optimal \emph{integer} branching factors and tree height, assuming equal privacy budgets at all levels. Finally, we describe general strategies for improving the private CDF estimates further, by combining multiple noisy estimates and by post-processing the estimates for consistency.

==> consistentsolution.tex <==
\label{sec:consistentsolution}
Our solution to the problem (O$^c$) is presented as Algorithm \ref{alg:optl1tree}.
\begin{algorithm}
	\caption{An optimal solution to (O$^c$)}
	\begin{algorithmic}[1]
		\Procedure {\textsc{OPT-$\ell_1$-Tree}}{$\mathcal{T}_m$, $M_\chi^\text{Lap}$}
		\State Set $\tilde{M}_{\chi(v_1)} = n$.
		\For{$i = 1: m-1$}
		\For{$(j_1,\ldots,j_i) = (1,\ldots,1):(n_1,\ldots,n_i)$} \label{step:sweep}
		\State Set $v\gets v_{1,j_1,\ldots,j_i}$ and $P(v) \gets  v_{1,j_1,\ldots,j_{i-1}}$.
		\State Set $\tilde{M}_{<\chi(v)}\gets \sum_{u = v_{1,j_1,j_2\ldots,r_i}: r_i<j_i} \tilde{M}_{\chi(u)}$.
		\If{$M_{\chi(v)}^\text{Lap}\leq 0$}
		\State Set $\tilde{M}_{\chi(v)} = 0$.
		\ElsIf{$M_{\chi(v)}^\text{Lap}\geq \tilde{M}_{\chi(P(v))} - \tilde{M}_{<\chi(v)}$}
		\State Set $\tilde{M}_{\chi(v)} = \tilde{M}_{\chi(P(v))} - \tilde{M}_{<\chi(v)}$.
		\Else
		\If{$j_i < n_i$}
		\State Set $\tilde{M}_{\chi(v)} = M_{\chi(v)}^\text{Lap}$.
		\Else
		\State Set $\tilde{M}_{\chi(v)} = \tilde{M}_{\chi(P(v))}^\text{Lap} - \tilde{M}_{<\chi(v)}$.
		\EndIf
		\EndIf
		\EndFor
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\label{alg:optl1tree}
\end{algorithm}
We mention that Algorithm \ref{alg:optl1tree} sets the $\tilde{M}_{\chi(v)}$ values for nodes $v$ in $\mathcal{T}_m$ recursively, exploring the tree in a breadth-first fashion, where at each level, we sweep over the nodes ordered according to the standard lexicographic order (see Step \ref{step:sweep}).
\begin{theorem}
	The solution $\tilde{M}_\chi$ in Algorithm \ref{alg:optl1tree} is optimal for the problem (O$^c$). 
\end{theorem}
\begin{proof}
	The proof proceeds by noting that the optimization problem (O$^c$) is convex in the variables $\{\tilde{M}_{\chi(v)}\}$. With each equation corresponding to node $v$ in Condition 1, we associate a Lagrange multiplier $\mu_v\geq 0$. With each equation corresponding to node $u$ in Condition 2, we associate a Lagrange multiplier $\lambda_u\geq 0$; in addition, we associate the Lagrange multiplier $\lambda_{v_1}$ for the constraint that is Condition 3. Let $\boldsymbol{\lambda}:= (\lambda_v:\ v \text{ in } \mathcal{T}_m)$ be the vector of Lagrange multipliers. We then construct the Lagrangian
	\begin{align*}
	\mathcal{L}(\tilde{M}_\chi, \boldsymbol{\lambda}, \boldsymbol{\mu})
	= \left\lVert \tilde{M}_\chi - M^\text{Lap}_\chi\right \rVert_1 + \sum_v \lambda_v\cdot&\left(\sum\limits_{u\in \psi(v)} \tilde{M}_{\chi(u)} - \tilde{M}_{\chi(v)}\right)\\
	 & - \sum_v \mu_v \tilde{M}_{\chi(v)}.
	\end{align*}
	In the above expression, we use the notation $\psi(v)$ to denote the collection of children of a node $v$ in $\mathcal{T}_m$. By standard arguments in convex optimization theory, we note that the KKT conditions are necessary for optimality \cite[Sec. 5.5.3]{boyd} of a solution to (O$^c$). \footnote{Here, subderivatives are used in place of standard derivatives, for non-differentiable convex functions.} We thus obtain that an optimal solution $\tilde{M}_\chi$ must satisfy, for all $v\neq v_1$:
	\begin{itemize}
		\item Stationarity:
		\begin{align*}
		0 &= \frac{\partial \mathcal{L}}{\partial \tilde{M}_{\chi(v)}}\\
		 &= \mathds{1}\{\tilde{M}_{\chi(v)}\geq M_{\chi(v)}^\text{Lap}\}-\mathds{1}\{\tilde{M}_{\chi(v)}< M_{\chi(v)}^\text{Lap}\}\\
		 &\ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ +\lambda_{P(v)} - \lambda_v - \mu_v.
		\end{align*}
	\item Complementary slackness:
	\[
	\lambda_v\cdot \left(\sum\limits_{u\in \psi(v)} \tilde{M}_{\chi(u)} - \tilde{M}_{\chi(v)}\right) = 0.
	\]
	\end{itemize}
The proof then proceeds by induction on the nodes $v$ in $\mathcal{T}_m$ in a breadth-first order, with the nodes at a given level being ordered in the lexicographic order. For the base case, consider the root node $v_1$. We set $\tilde{M}_{\chi(v_1)} = n$, thereby satisfying complementary slackness; the value $\lambda_{v_1}$ is then picked to satisfy the KKT condition \begin{align*}
	\lambda_{v_1} = \mathds{1}\{\tilde{M}_{\chi(v_1)}\geq M_{\chi(v_1)}^\text{Lap}\}-\mathds{1}\{\tilde{M}_{\chi(v_1)}< M_{\chi(v_1)}^\text{Lap}\} = 1,
\end{align*}
by the fact that we define $M_{\chi(v_1)}^\text{Lap} = n$.
Now, assume that the Lagrangian multipliers $\mu_u, \lambda_u\geq 0$ have been assigned for all nodes $u$ that occur before node $v$ in the order above. For node $v$, we follow the procedure below:
\begin{enumerate}
	\item $M_{\chi(v)}^\text{Lap}\leq 0$: In this case, we set $\tilde{M}_{\chi(v)} = 0$, $\lambda_v = 0$, and $\mu_v = 1+\lambda_{P(v)}\geq 0$.
	\item $M_{\chi(v)}^\text{Lap}\geq \tilde{M}_{\chi(P(v))} - \tilde{M}_{<\chi(v)}$: In this case, we set $\tilde{M}_{\chi(v)} = \tilde{M}_{\chi(P(v))} - \tilde{M}_{<\chi(v)}$, thereby satisfying complementary slackness, and 
	\item 
\end{enumerate}
\end{proof}

==> consistentsolution2.tex <==
\label{sec:consistentsolution}

==> error-bounds.tex <==
\label{sec:errorbounds}

==> l1-post-process.tex <==
\label{sec:post-process}
In this section, we shift our focus to the $\ell_1$-error and seek to process (potentially differentially private) estimates of the CDF $\mathbf{F}$ (see \eqref{eq:cdf}), obtained via a tree-based mechanism, into an estimate that satisfies natural \emph{consistency} requirements; the term ``consistency" here simply refers to standard desirable properties of the statistic of interest, which in our case is the CDF. In our first approach, we extend and explicitly solve an instance of a ``tree-based'' consistency problem that was first introduced in \cite{histhay} for the $\ell_2$-error and then considered in \cite{histml} under the $\ell_1$-error, both in the context of histogram estimation. As we shall see, any consistent tree-based solution for histogram estimation is also a consistent tree-based solution for CDF estimation. While \cite{histml} discussed numerical algorithms for solving such a problem, we provide an explicit, analytical solution. In our second approach, we ignore the fact that the original estimates of the CDF $\mathbf{F}$ arise from a tree-based mechanism and seek to simply output a (CDF-)consistent estimate of an existing estimate of $\mathbf{F}$.%we shall make these requirements more precise, in what follows.

\subsection{A Tree-Based $\ell_1$-Consistency Problem}

Fix a height $m\geq 1$ of the tree $\mathcal{T}_m$ defined in Section \ref{sec:tree} and consider a level-uniform tree-based mechanism $\mathbf{F}^\text{tree}(\mathbf{n},\boldsymbol{\varepsilon};\cdot)$, obtained via the vector $M_\chi^\text{Lap}$ in \eqref{eq:mchilap} \footnote{The post-processing steps discussed in this section continue to hold for mechanisms where the values $M_{\chi(v)}^\text{Lap}$ are computed potentially arbitrarily and not necessarily according to \eqref{eq:mchi}.}. We mention that the choice of the parameters $\mathbf{n}, \boldsymbol{\varepsilon}$ is arbitrary and not necessarily according to any notion of optimality as in the previous sections. We call a  vector $\tilde{M}_\chi:=\left(\tilde{M}_{\chi(v)}:\ v\text{ is a node of $\mathcal{T}_m$}\right)$ of estimates of $\chi:= \left(\chi(v):\ v\text{ is a node of $\mathcal{T}_m$}\right)$ as consistent if the following two conditions hold:
\begin{enumerate}
	\item $\tilde{M}_{\chi(v)}\geq 0$, for all nodes $v\neq v_1$ in $\mathcal{T}_m$ and
	\item $\sum\limits_{\substack{v:\ \text{$v$ child}\\ \text{ of $u$}}} \tilde{M}_{\chi(v)} \leq \tilde{M}_{\chi(u)}$, for all nodes $u\neq v_1$ in $\mathcal{T}_m$.
	\item $\tilde{M}_{v_1} = n$.
\end{enumerate}
Condition 1) above simply requires that estimates of the (non-negative) counts corresponding to any sub-interval $\mathcal{I}(v)$ be non-negative.  Condition 2) requires that the sum of the estimates of the counts of child nodes never exceed the estimate at the parent node -- this condition is natural in the context of approximate CDF computation via strategies such as that in \eqref{eq:cdfcompute}, as it ensures that the resultant CDF estimate is non-decreasing\footnote{We add that Condition 2) with an equality instead of an inequality has been considered as part of post-processing steps for consistent \emph{histogram} release \cite{histhay, histml}.}. Condition 3) states that the estimate at the root node of $\mathcal{T}_m$ be equal to the (publicly known) value $n = \chi(v_1)$.

We let $\mathcal{C}_m$ denote the set of vectors $\tilde{M}_\chi$ that satisfy the consistency constraints in Conditions 1)--3) above. In this work, as mentioned in the Introduction, we are interested in ``post-processing'' the noisy vector of estimates $M^\text{Lap}_\chi$ obtained via \eqref{eq:mchi} into the ``closest, consistent'' estimate $\tilde{M}_\chi$. More formally, we are interested in the following optimization problem:
\begin{align}
	&{\text{minimize}}\quad \left\lVert \tilde{M}_\chi - M^\text{Lap}_\chi\right \rVert_1\notag\\
	&\text{subject to:}\ \  \tilde{M}_\chi\in \mathcal{C}_m. \tag{O$^c$} \label{eq:optconsistency}
\end{align}
The vector of estimates $\tilde{M}_\chi$ is used for computing an estimate $\tilde{\mathbf{F}}^\text{tree}$ as in Definition \ref{def:cdftree} and \eqref{eq:mchilap}, which is then released to the client for use in downstream applications. 

As mentioned earlier, variants of this problem have been considered in past work, in the context of the release of consistent, differentially private histograms. In particular, \cite{histhay} sought to minimize the \emph{$\ell_2$-error} between $\tilde{M}_\chi$ and $\chi$ subject to Condition 2) being met with equality, and obtained an explicit, analytical expression for $\tilde{M}_\chi$ by relating the problem to isotonic regression. In our work, we focus on the $\ell_1$-error since it is an error metric that arises naturally in maximum likelihood estimation of the parameters of a Laplace distribution, as observed in \cite{histml}. However, \cite{histml} only considered Conditions 1) and 2) above, with Condition 2) being an equality constraint, and further, provided a numerical approach to solving the problem using the Alternating Direction Method of Multipliers (ADMM) \cite{admm}. In our work, we provide an \emph{explicit}, simple solution to the optimization problem \eqref{eq:optconsistency} in Section \ref{sec:consistentsolution}. 
%In Section \ref{sec:errorbounds}, we briefly discuss how imposing consistency requirements can also help improve the $\ell_1$-error $E_1(\tilde{\mathbf{F}}^\text{tree}) = \left\lVert \tilde{M}_\chi - \chi\right \rVert_1$ compared to $E_1(\mathbf{F}^\text{tree})$, in some simple, special cases.

\subsubsection{Explicit Consistent Solution}
\input{consistentsolution.tex}
\subsubsection{Error Bounds for Consistent CDFs}
\input{error-bounds.tex}

==> results.tex <==
\label{sec:results}
\subsection{Setup}

%\begin{figure*}[]
%	\centering
%	\includegraphics[width=0.8\linewidth]{grouping.png}
%	\caption{Plots comparing $E_\text{RMSE}$ and $E_\text{MAE}$ for the \textsc{Array-Averaging}, \textsc{Levy}, and \textsc{Quantile} algorithms, under the two grouping strategies. For the \textsc{Levy} algorithm, we fix $\gamma = 0.2$, and for the \textsc{Quantile} algorithm, we use the \textsc{FixedQuantile} subroutine.}
%	\label{fig:group}
%\end{figure*}

%Prajjwal: We compare our algorithms with two approaches. The first approach is a baseline which involves the naive use of laplace mechanism in which laplace noise is added with sensitivity $\frac{(b-a)m^{*}}{\sum_{i=1}^{n}m_{i}}$ where $m^{*}$ is the maximum number of samples contributed by any user. Thus the final estimate $\mu_{base1}$ is given by :
%
%\begin{equation}
%	\mu_{base1} = \frac{\sum_{i=1}^{n} \sum_{j=1}^{m_{i}} x_{j}}{\sum_{k=1}^{n} m_{k}} + Lap(\frac{(b-a)m^{*}}{\sum_{p=1}^{n}m_{p}\epsilon})
%\end{equation}
%
%The second approach is the algorithm proposed by Levy et. al in [Lev+21]. Their algorithm considers the case in which all users contribute same number of samples. So in order to fit their approach to out setting, we modify and extend their algorithm with \textsc{WrapAroundGrouping}. Note that their approach assumes samples drawn i.i.d from a sub-Gaussian distribution, and hence is not expected to give optimal results in a non-i.i.d setting. Additionally \textsc{BestFitGrouping} cannot be used in conjunction with their approach as the subsequent "Median of Means" algorithm for interval calculation requires all samples groups to be completely filled in order to exploit the concentration property contained by the coarse mean $\mu_{c}$ and $\tau$. $\tau$ is a constant which is given by $\sigma \sqrt{ \frac{2}{l} log(\frac{2k}{\gamma} ) }$. The interval estimated by [Lev+21] is given by $\mathcal{I}_{Levy}$[$\bar{\mu} - 1.5\tau$, $\bar{\mu} + 1.5\tau$] where $\bar{\mu}$ is the private median of means. Thus, the sensitivity of the mean of $Z_{i}$ after projecting them to this interval is limited to $\frac{3\tau}{k}$. Thus the final estimate using Levy et al.'s approach is given by:
%
%\begin{equation}
%	\mu_{levy} = \frac{\sum_{i=0}^{k}\prod_{\mathcal{I}_{levy}}Z_{i}}{k} + Lap(\frac{12\tau}{k\epsilon})
%\end{equation}
%
%For comparing our algorithm with their approach,  we set $\gamma = 0.2$ which corresponds to the probability that any mean $Z_{i}$ would lie beyond the interval returned by the algorithm. Since in our algorithm, $\alpha$ and $\beta$ correspond to the $10^{th}$ and $90^{th}$ quantiles respectively, we are effectively winsorizing 20\% of $Z_{i}$ which makes the comparison fair with [Lev+21] with $\gamma = 0.2$.


{In \cite{dp_spcom}, we evaluated our algorithms on two types of datasets: 1) a real-world ITMS dataset $\mathcal{C}$ containing non-i.i.d. speed values and 2) a synthetic dataset $\mathcal{D}$ containing i.i.d. samples drawn using insights from the ITMS data. We ran each private mean estimation algorithm $10^4$ times and tested the accuracy of our algorithms for privacy loss $\epsilon\in [0.5,2]$.}

We used the mean absolute error (or MAE) metric, $E_\text{MAE}(\mathcal{C}) = 10^{-4}\cdot {{\sum_{i=0}^{10^4} \left \lvert M^{(i)}(\mathcal{C}) - \mu(\mathcal{C})\right \lvert}}$, to evaluate the performance of the algorithms. Here, for $i\in [10^4]$, $M^{(i)}(\mathcal{C})$ is the result of running each algorithm $M$ in Section \ref{sec:alg} on  $\mathcal{C}$ at iteration $i$, and $\mu:=\mu(\mathcal{C})$ is the true sample mean. Since, for $Z\sim \text{Lap}(b)$, we have $\E[|Z|] = b$, we simply used $E_\text{MAE}(\mathcal{C}) = \Delta_f/\varepsilon$ for \textsc{Baseline}.
% How to write the percentile formula ?

\subsection{Experimental Results}
We refer the reader to Appendix \ref{app-numerics} for details on the ITMS dataset $\mathcal{C}$ and for plots of the performance of our algorithms on the ITMS data, which show that \textsc{Baseline} performs uniformly poorer than all other algorithms.

Next, we artificially generated\footnote{An interesting direction for future study is the $\epsilon$-differentially private generation of synthetic data that preserves some statistics of the base dataset (see \cite{vershynindp} and references therein).} a large dataset ${\mathcal{D}}$ using insights from the ITMS dataset. Let the number of users in $\mathcal{D}$ be $\widehat{L}$ and let the number of samples per user be $\{\widehat{m}_\ell\}_{\ell\in [\widehat{L}]}$.
%In particular, let $\widehat{L}$ denote the number of users and $\widehat{m_\ell}$, for $\ell \in [\widehat{L}]$ denote the number of samples contributed by user $\ell$. Recall that $L$ and $\{m_\ell: \ell \in [L]\}$ denote the number of users and the collection of the number of samples per user for the original ITMS dataset. 
We generated i.i.d. speed samples $\left\{\widehat{S}_j^{(\ell)}: \ell \in [\widehat{L}], j\in [\widehat{m_\ell}]\right\}$, where for any $\ell, j$, we have $\widehat{S}_j^{(\ell)}\sim \Pi_{[0,U]}(X)$, where $X\sim \mathcal{N}(\mu,\sigma^2)$. Here, 
$
\sigma^2 = \sigma^2(\mathcal{C}) = \frac{1}{\sum_{\ell=1}^{L}{m_\ell}}\cdot \sum_{\ell=1}^L \sum_{j=1}^{m_\ell}\left(S_j^{(\ell)}-\mu\right)^2
$
is the true variance of the ITMS dataset. 

%Note that the  random variable $\widehat{S}_j^{(\ell)}$ obeys
%$
%	\Pr\left[\hat{S}_j^{(\ell)} = 0\right] = Q\left(\frac{\mu(\mathcal{D})}{\sigma(\mathcal{D})}\right)\ \text{and}\ \Pr\left[\hat{S}_j^{(\ell)} = U\right] = Q\left(\frac{U-\mu(\mathcal{D})}{\sigma(\mathcal{D})}\right).
%$

We consider two settings, for a fixed positive integer $\lambda$.
\begin{enumerate}
	\item \textbf{Sample scaling}: Here, we set $\widehat{L} = L$ and $\widehat{m}_\ell = \lambda \cdot m_\ell$, for all $\ell\in [\widehat{L}]$. In this case, $\widehat{m}^\star := \max_{\ell\in [\widehat{L}]} \widehat{m}_\ell = \lambda\cdot m^\star$. 
	\item \textbf{User scaling}: Here, we set $\widehat{L} = \lambda\cdot L$ and for each $i\in [\lambda]$, we let $\widehat{m}_{\lambda\cdot(\ell-1)+i} = m_\ell$,  for all $\ell\in [{L}]$. Here, $\widehat{m}^\star = m^\star$.
\end{enumerate}
Plots for the performance of our algorithms under \textbf{sample scaling} and \textbf{user scaling} can be found in {Appendix} \ref{app-numerics}, with $\lambda$ set to $10$. 
Figure \ref{fig:sample-scale} there for \textbf{sample scaling} shows that \textsc{Baseline} performs worse than the other algorithms, as expected. However, interestingly, the \textsc{Levy} algorithm (with $\gamma = 0.2$) outperforms than all other algorithms. 
%The justification for the relative superior performance of \textsc{Levy} in the sample scaling setting 
%can be found in Appendix \ref{app-sample-scaling}.

%is as follows. First, observe that in \textsc{Levy}, we have that 
%%$
%%\widehat{m}_\text{UB} = \text{argmax}_{m} \frac{\sum_{\ell=1}^{L}\min \left  \{10\cdot m_{\ell}, m \right \}}{\sqrt{m}}.
%%$
%$\widehat{m}_\text{UB} = 10\cdot m_\text{UB}$ solves \eqref{eq:uboptim}, where $m_\text{UB}$ was the length of the arrays used in the absence of sample scaling. Furthermore, the number of arrays $\widehat{\overline{K}}$ obtained using \textsc{BestFit} grouping equals $\overline{K}$. Hence,
%$
%\Delta_{f_\text{Levy}}(\widehat{m}_\text{UB}) = \frac{3U}{\overline{K}}\sqrt{\frac{\log (2\overline{K}/\gamma)}{20m_\text{UB}}},
%$
%which is a factor $1/\sqrt{10}$ smaller than the user-level sensitivity without scaling. 
%In general, when the number of samples per user is scaled by a factor of $\lambda>1$, we get a multiplicative factor of $1/\sqrt{\lambda}$ improvement in the user-level sensitivity, and hence in the standard deviation of the noise added, thereby improving performance. 
%{
%In contrast, the sensitivities for \textsc{Baseline} and \textsc{Array-Averaging} remain unchanged from the corresponding values without sample scaling.} 

%Based on the analysis in Appendix \ref{app-sample-scaling}, in general, when the dataset contains a large number of samples per user, we recommend using \textsc{Levy}.

Figure \ref{fig:user-scale} in Appendix \ref{app-numerics} for \textbf{user scaling} shows that the \textsc{FixedQuantile} subroutine outperforms all the other algorithms. Furthermore, \textsc{Array-Averaging} performs second-best. We reiterate that we used $m_\text{UB} = m_{\text{UB}}^{(L)}$ (see \eqref{eq:uboptim}) for \textsc{Array-Averaging} as well, to maintain uniformity. 

In the next section, we provide theoretical justification for the performance trends we observe on large datasets.
%We justify these performance trends in Appendix \ref{app-user-scaling}.

%Figure \ref{fig:user-scale} for \textbf{user scaling} shows that the \textsc{FixedQuantile} subroutine outperforms all the other algorithms. We mention here that we use $m_\text{UB}$ as in \eqref{eq:uboptim} for \textsc{Array-Averaging} as well, to maintain uniformity. To justify the performance trends, note that for \textsc{Levy}, $\tau$ (and hence $\Delta_{f_\text{Levy}}$) increases (logarithmically) with the number of users. This implies that when  the number of users are sufficiently large, the computed interval $[a,b]$ will be equal to the entire interval $(0,U]$. Next, for \textsc{$\varepsilon$-DependentQuantile}, note that since $\epsilon\geq 0.5$, we have that the interval $[a',b']$ excludes $\left \lfloor 4/\varepsilon \right \rfloor \leq 8$ outlier speed samples, suggesting that for typical datasets with a large number of users, $b'-a'\approx U$. In comparison, the \textsc{FixedQuantile} subroutine eliminates a much larger number of data samples in the computation of $[a',b']$, implying that the amount of noise added in this case is low. 

%Based on the analysis in Appendix \ref{app-user-scaling}, for datasets with a large number of users, we recommend using \textsc{FixedQuantile}.

%\begin{figure}
%	\centering
%	\subfloat[]
%	{
%		\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_NS+BS.png}
%		\caption{95th percentile error vs Epsilon graph}
%		\label{fig:itmscompare}
%	}
%	\subfloat[]
%	{
%		\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_US.png}
%		\caption{95th percentile error vs Epsilon graph}
%		\label{fig:userscale}
%	}
%	\caption{ Two foo figures. }
%	\label{fig:foo}
%\end{figure}


%\begin{figure}
%	\centering
%	\begin{tabular}{cc}
%		%\subfloat[A]{\includegraphics[width=0.5\linewidth]{ConcentrationAlgoComparisonBestFit_NS+BS.png}} & 
%		\subfloat[Comparison of algorithms under sample scaling]{\includegraphics[width=0.4\linewidth]{samplescaling.png}} &
%		\subfloat[Comparison of algorithms under user scaling]{\includegraphics[width=0.4\linewidth]{optimizedquantile.png}}
%	%	\subfloat[C]{\includegraphics[width=0.5\linewidth]{ConcentrationAlgoComparisonBestFit_SynthUser+BS.png}} & 
%		\\
%	\end{tabular}
%	\caption{Many figures}
%\end{figure}




%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_NS+BS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{fig:itmscompare}
%\end{figure}

%Do we need this? \begin{figure}[!h]
%	\centering
%	\includegraphics[width=3.4in]{ConcentrationAlgoComparisonBestFit_SS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_US.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{fig:userscale}
%\end{figure}

%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_SynthUser+BS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}
%
%\begin{figure}[!h]
%	\centering
%	\includegraphics[width=0.7\linewidth]{ConcentrationAlgoComparisonBestFit_Synth+BS.png}
%	\caption{95th percentile error vs Epsilon graph}
%	\label{perc95}
%\end{figure}
